SpeqNets: Sparsity-aware Permutation-equivariant Graph Networks

While (message-passing) graph neural networks have clear limitations in approximating permutation-equivariant functions over graphs or general relational data, more expressive, higher-order graph neural networks do not scale to large graphs. They either operate on $k$-order tensors or consider all $k$-node subgraphs, implying an exponential dependence on $k$ in memory requirements, and do not adapt to the sparsity of the graph. By introducing new heuristics for the graph isomorphism problem, we devise a class of universal, permutation-equivariant graph networks, which, unlike previous architectures, offer a fine-grained control between expressivity and scalability and adapt to the sparsity of the graph. These architectures lead to vastly reduced computation times compared to standard higher-order graph networks in the supervised node- and graph-level classification and regression regime while significantly improving over standard graph neural network and graph kernel architectures in terms of predictive performance.

==> name.tex <==
SpeqNets: SpeqNets: Sparsity-aware Permutation-equivariant Graph Networks

Christopher Morris (McGill University and Mila), joint work with Gaurav Rattan, Sandra Kiefer (RWTH Aachen), and Siamak Ravanbakhsh (McGill University and Mila)

Standard graph neural networks have clear limitations in approximating permutation-equivariant functions over graphs, i.e., their expressive power is bounded the 1-WL [1,2]. Hence, more expressive, higher-order graph neural networks have recently emerged, e.g. [1,3], which overcome these limitations. However, they either operate on $k$-order tensors or consider all $k$-node subgraphs, implying an exponential dependence on $k$ in memory requirements, and do not adapt to the sparsity of the graph. In [4], we introduce a new class of heuristics for the graph isomorphism problem, the (k,s)-WL, which offers a more fine-grained control between expressivity and scalability and adapts to the sparsity of the graph. Essentially, the algorithm is a variant of the local k-WL [4] but only considers specific tuples to avoid the exponential memory complexity of the k-WL. Concretely, the algorithm only considers k-tuples or subgraphs on k nodes with the most s connected components, effectively exploiting the potential sparsity of the underlying graph. On the theoretical side, we show how varying k and s leads to a tradeoff between scalability and expressivity, 

We derive a new hierarchy of permutation-equivariant graph neural networks based on these combinatorial insights, reaching universality in the limit. These architectures vastly reduce computation times compared to standard higher-order graph networks in the supervised node- and graph-level classification and regression regime, significantly improving standard graph neural network and graph kernel architectures in predictive performance.

==> sparser_wl (2)/figures/g.tex <==
\begin{tikzpicture}

\tikzset{line/.style={draw,thick}}
\tikzset{arrow/.style={line,->,>=stealth}}
\tikzset{node/.style={circle,inner sep=0pt,minimum width=15pt}}

\node[line,node,fill=gray] (x1)  at (0.75,  0.00) {};
\node[line,node,fill=gray] (x2)  at (1.25,  0.75) {};
\node[line,node,fill=gray] (x3)  at (2.25,  0.75) {};
\node[line,node,fill=gray] (x4)  at (2.75,  0.00) {};
\node[line,node,fill=gray] (x5)  at (2.25, -0.75) {};
\node[line,node,fill=gray] (x6)  at (1.25, -0.75) {};
\node[line,node,fill=gray] (x7)  at (3.75,  0.00) {};
\node[line,node,fill=gray] (x8)  at (4.25,  0.75) {};
\node[line,node,fill=gray] (x9)  at (5.25,  0.75) {};
\node[line,node,fill=gray] (x10) at (5.75,  0.00) {};
\node[line,node,fill=gray] (x11) at (5.25, -0.75) {};
\node[line,node,fill=gray] (x12) at (4.25, -0.75) {};

\path[line] (x1) to (x2);
\path[line] (x2) to (x3);
\path[line] (x3) to (x4);
\path[line] (x4) to (x5);
\path[line] (x5) to (x6);
\path[line] (x6) to (x1);
\path[line] (x4) to (x7);
\path[line] (x7) to (x8);
\path[line] (x8) to (x9);
\path[line] (x9) to (x10);
\path[line] (x10) to (x11);
\path[line] (x11) to (x12);
\path[line] (x12) to (x7);

\end{tikzpicture}

==> sparser_wl (2)/figures/g_map.tex <==
\begin{tikzpicture}

\tikzset{line/.style={draw,thick}}
\tikzset{arrow/.style={line,->,>=stealth}}
\tikzset{node/.style={circle,inner sep=0pt,minimum width=15pt}}

\node[] (x1)  at (0.75,  0.00) {\large\textbf{\dots}};
\node[line,node,fill=blue] (x2)  at (1.25,  0.75) {};
\node[line,node,fill=green] (x3)  at (2.25,  0.75) {};
\node[line,node,fill=yellow] (x4)  at (2.75,  0.00) {};
\node[line,node,fill=pink] (x5)  at (2.25, -0.75) {};
\node[line,node,fill=gray] (x6)  at (1.25, -0.75) {};
\node[line,node,fill=purple] (x7)  at (3.75,  0.00) {};
\node[line,node,fill=white] (x8)  at (4.25,  0.75) {};
\node[line,node,fill=olive] (x9)  at (5.25,  0.75) {};
\node[] (x10) at (5.75,  0.00) {\large\textbf{\dots}};
\node[line,node,fill=lime] (x11) at (5.25, -0.75) {};
\node[line,node,fill=orange] (x12) at (4.25, -0.75) {};

\path[line] (x1) to (x2);
\path[line] (x2) to (x3);
\path[line] (x3) to (x4);
\path[line] (x4) to (x5);
\path[line] (x5) to (x6);
\path[line] (x6) to (x1);
\path[line] (x4) to (x7);
\path[line] (x7) to (x8);
\path[line] (x8) to (x9);
\path[line] (x9) to (x10);
\path[line] (x10) to (x11);
\path[line] (x11) to (x12);
\path[line] (x12) to (x7);

\node[] (xx1)  at (8.75,   0.00) {\large\textbf{\dots}};
\node[line,node,fill=blue] (xx2)  at (9.25,   0.75) {};
\node[line,node,fill=green] (xx3)  at (10.25,   0.75) {};
\node[line,node,fill=yellow] (xx4)  at (11.25,   0.50) {};
\node[line,node,fill=purple] (xx5)  at (11.25,  -0.50) {};
\node[line,node,fill=white] (xx6)  at (10.25,  -0.75) {};
\node[line,node,fill=olive] (xx7)  at (9.25,  -0.75) {};
\node[line,node,fill=pink] (xx8)  at (12.25,  0.75) {};
\node[line,node,fill=gray] (xx9)  at (13.25,  0.75) {};
\node[] (xx10) at (13.75,  0.00) {\large\textbf{\dots}};
\node[line,node,fill=lime] (xx11) at (13.25, -0.75) {};
\node[line,node,fill=orange] (xx12) at (12.25, -0.75) {};

\path[line] (xx1) to (xx2);
\path[line] (xx2) to (xx3);
\path[line] (xx3) to (xx4);
\path[line] (xx4) to (xx5);
\path[line] (xx5) to (xx6);
\path[line] (xx6) to (xx7);
\path[line] (xx7) to (xx1);
\path[line] (xx4) to (xx8);
\path[line] (xx8) to (xx9);
\path[line] (xx9) to (xx10);
\path[line] (xx10) to (xx11);
\path[line] (xx11) to (xx12);
\path[line] (xx12) to (xx5);

\end{tikzpicture}

==> sparser_wl (2)/figures/h.tex <==
\begin{tikzpicture}

\tikzset{line/.style={draw,thick}}
\tikzset{arrow/.style={line,->,>=stealth}}
\tikzset{node/.style={circle,inner sep=0pt,minimum width=15pt}}



\node[line,node,fill=gray] (x1)  at (0.75,   0.00) {};
\node[line,node,fill=gray] (x2)  at (1.25,   0.75) {};
\node[line,node,fill=gray] (x3)  at (2.25,   0.75) {};
\node[line,node,fill=gray] (x4)  at (3.25,   0.50) {};
\node[line,node,fill=gray] (x5)  at (3.25,  -0.50) {};
\node[line,node,fill=gray] (x6)  at (2.25,  -0.75) {};
\node[line,node,fill=gray] (x7)  at (1.25,  -0.75) {};
\node[line,node,fill=gray] (x8)  at (4.25,  0.75) {};
\node[line,node,fill=gray] (x9)  at (5.25,  0.75) {};
\node[line,node,fill=gray] (x10) at (5.75,  0.00) {};
\node[line,node,fill=gray] (x11) at (5.25, -0.75) {};
\node[line,node,fill=gray] (x12) at (4.25, -0.75) {};

\path[line] (x1) to (x2);
\path[line] (x2) to (x3);
\path[line] (x3) to (x4);
\path[line] (x4) to (x5);
\path[line] (x5) to (x6);
\path[line] (x6) to (x7);
\path[line] (x7) to (x1);
\path[line] (x4) to (x8);
\path[line] (x8) to (x9);
\path[line] (x9) to (x10);
\path[line] (x10) to (x11);
\path[line] (x11) to (x12);
\path[line] (x12) to (x5);

\end{tikzpicture}

==> sparser_wl (2)/figures/u.tex <==
\begin{tikzpicture}[node distance = {.5cm}, v/.style = {draw, circle}, minimum size=25pt,every node/.style={inner sep=0pt,outer sep=0}]
  \node (a) [v] {$a_{(0,a)}$};
  \node (b) [v, below  = .4cm of a] {$c_{(1,a)}$};
\node (c) [v, below right = 1.cm of a] {$b_{(1,a)}$};
\node (d) [v, below left = 1.cm of a] {$d_{(1,a)}$};

\node (e) [v, below =  .4cm of d] {$a_{(2,d)}$};
\node (f) [v, below left =1.0cm of d] {$b_{(2,d)}$};
%
\node (g) [v, below = .4cm of b] {$a_{(2,c)}$};
%
\node (i) [v, below  =  .4cm of c] {$a_{(2,b)}$};
\node (j) [v, below right = 1.0cm of c] {$d_{(2,b)}$};

\draw[->] (a) to node[above] {} (b);
\draw[->] (a) to node[above] {} (c);
\draw[->] (a) to node[above] {} (d);


\draw[->] (d) to node[above] {} (e);
\draw[->] (d) to node[above] {} (f);
\draw[->] (b) to node[above] {} (g);

\draw[->] (c) to node[above] {} (i);
\draw[->] (c) to node[above] {} (j);
\end{tikzpicture}

==> sparser_wl (2)/figures/v.tex <==
\begin{tikzpicture}[node distance = {.5cm}, v/.style = {draw, circle},  minimum size=25pt,every node/.style={inner sep=0pt,outer sep=0}]
  \node (a) [v] {$a$};
  \node (b) [v, left = of a] {$b$};
  \node (c) [v, right = of a] {$c$};
  \node (d) [v, above = of a] {$d$};


  \draw (a) to node[above] {} (c);
  \draw (a) to node[above] {} (b);
  \draw (a) to node[above] {} (d);

  \draw (d) to node[above] {} (b);
\end{tikzpicture}

==> sparser_wl (2)/name.tex <==
SpeqNets: SpeqNets: Sparsity-aware Permutation-equivariant Graph Networks

Christopher Morris (McGill University and Mila), joint work with Gaurav Rattan, Sandra Kiefer (RWTH Aachen), and Siamak Ravanbakhsh (McGill University and Mila)

Standard graph neural networks have clear limitations in approximating permutation-equivariant functions over graphs, i.e., their expressive power is bounded the 1-WL [1,2]. Hence, more expressive, higher-order graph neural networks have recently emerged, e.g. [1,3], which overcome these limitations. However, they either operate on $k$-order tensors or consider all $k$-node subgraphs, implying an exponential dependence on $k$ in memory requirements, and do not adapt to the sparsity of the graph. In [4], we introduce a new class of heuristics for the graph isomorphism problem, the (k,s)-WL, which offers a more fine-grained control between expressivity and scalability and adapts to the sparsity of the graph. Essentially, the algorithm is a variant of the local k-WL [4] but only considers specific tuples to avoid the exponential memory complexity of the k-WL. Concretely, the algorithm only considers k-tuples or subgraphs on k nodes with the most s connected components, effectively exploiting the potential sparsity of the underlying graph. On the theoretical side, we show how varying k and s leads to a tradeoff between scalability and expressivity, 

We derive a new hierarchy of permutation-equivariant graph neural networks based on these combinatorial insights, reaching universality in the limit. These architectures vastly reduce computation times compared to standard higher-order graph networks in the supervised node- and graph-level classification and regression regime, significantly improving standard graph neural network and graph kernel architectures in predictive performance.
